SOCIA-$\nabla$: Textual Gradient Meets Multi-Agent Orchestration for Automated Simulator Generation

In this paper, we present SOCIA-$\nabla$, a diagnosis-driven multi-agent framework for automated simulator-code construction. SOCIA-$\nabla$ iteratively refines executable simulator code within a textual computation graph, where LLM-driven agents synthesize, execute, evaluate, diagnose, and repair simulators. A grounded simulator blueprint attributes behavioral residuals to candidate mechanisms and their spatial or interaction contexts, which are then converted into localized textual repair signals with history-aware memory and constraint projection. We evaluate SOCIA-$\nabla$ on the real-world LLMob personal-mobility benchmark and a controlled semi-synthetic geo-social mask-adoption benchmark. Across in-distribution simulation, out-of-distribution what-if generation, and geo-social diffusion, SOCIA-$\nabla$ achieves the strongest overall simulator fidelity. SOCIA-$\nabla$'s code and data are publicly available at https://github.com/cruiseresearchgroup/SOCIA-Nabla.

==> latex/chapter/1_intro_old.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=1.0\textwidth]{latex/figure/socia_gradient.png} 
\caption{Overview of \socia. A multi-agent textual computation graph takes task brief and input data, synthesizes simulator code, executes it, and evaluates loss; the loss is converted into textual gradients that drive code optimization. Right: three representative applications illustrating alignment of simulated outputs with real observables.}
\label{fig:gradient}
% \vspace{-1em}
\end{figure*}

Building simulators is a research hotspot because they offer a low-cost, reproducible in-silico sandbox for controlled intervention and ``what-if” analysis, while enabling researchers to probe emergent outcomes under shifts and unseen regimes~\cite{bonabeau2002agent,cohen2017scientific,alves2023policy}.
By design, simulators span two paradigms: \emph{policy-oriented aggregate (system-dynamics / compartmental) models}, which summarize populations through equations over aggregated state variables, and \emph{agent-based / microsimulation models}, which follow heterogeneous decision units and their interactions to capture fine-grained dynamics~\cite{van1998agent,mitton2000microsimulation,macal2005tutorial,howick2024framework}. These approaches arise across cyber, physical, and social (CPS) domains~\cite{DBLP:journals/epjds/RenTSCS18,DBLP:journals/tkde/RenTSCCS18,DBLP:journals/tosn/KaurSRCTS20,DBLP:journals/access/PasandidehPG22,mcculloch2022calibrating}, making controlled, repeatable cross-domain experimentation feasible.

Regardless of form, simulators share a universal medium: \textbf{executable code}. In practice, a simulator is only useful when its rules, interfaces, and data flows are embodied in code that can be run, evaluated, and calibrated~\cite{kennedy2001bayesian,law2007simulation,grimm2020odd}. This observation motivates a pragmatic goal: if we could automate the construction of high-fidelity, extrapolatable simulator code with minimal expert effort, we would substantially lower the cost of building CPS simulators for computer scientists, sociologists, and domain practitioners.

Existing pathways only partially meet this bar. \emph{Manual, expert-built simulators}~\cite{zhang2025socioverse,DBLP:journals/corr/abs-2502-08691,DBLP:journals/corr/abs-2502-18712,jiawei2024large,yang2024oasis,tang2024gensim,yan2024opencity} are accurate but expensive to produce and maintain. \emph{Description-driven systems}—for example, YuLan-OneSim~\cite{wang2025yulan}, which converts natural-language scenario descriptions into code using ODD protocol~\cite{grimm2010odd} and behavior graphs—reduce coding burden but do not, by themselves, provide an inner loop for \emph{data calibration} of the generated programs. At the other end, recent \emph{automatic frameworks} such as G-Sim~\cite{DBLP:journals/corr/abs-2506-09272} pair LLM-proposed designs with simulation-based inference, showing promising alignment to observed data; however, these efforts have largely focused on aggregate models and may not readily extend to highly heterogeneous, micro-level simulators.

In parallel, \emph{multi-agent code generation} has advanced rapidly: CAMEL~\cite{li2023camel}, ChatDev~\cite{qian2023chatdev}, AgentCoder~\cite{huang2023agentcoder}, AutoGen~\cite{harper2024autogenesisagentselfgeneratingmultiagentsystems}, and AI Scientist-v2~\cite{yamada2025ai} stage specialized LLM agents to propose, test, and refine software or to conduct scientific experiments. These frameworks demonstrate compelling task decomposition and collaboration patterns, but they are typically \emph{prompt-sensitive, hand-tuned, and not designed for simulator construction or data calibration}—their agent protocols and success criteria are not embedded in a loss-compiled optimization view, and they seldom close the loop from execution metrics back to targeted code repair.

To overcome these challenges, we introduce \textbf{\socia} (Simulation Orchestration for Computational Intelligence with Agents), an end-to-end multi-agent framework that treats simulator building as \emph{instance optimization over code} within a \textbf{textual computation graph}. \socia defines specialized agents for data analysis, code generation, execution, evaluation, and feedback, and \emph{embeds each agent as a node} in a directed textual computation graph that carries both textual artifacts (code, logs, critiques) and numeric signals (metrics). A centralized workflow manager orchestrates \emph{forward execution} (generate code $\rightarrow$ run simulator $\rightarrow$ compute validation loss and constraint checks) and \emph{backward repair} (route \emph{textual gradients}—loss-aligned, natural-language critiques—toward the responsible upstream code components). The optimizer uses \emph{momentum} (history-aware aggregation of critiques) and \emph{projected gradient descent (PGD)–style projection} (constraint-aware repair to preserve compilability and schema conformance) to stabilize long-horizon edits. Human-in-the-loop (HITL) is employed for task-spec confirmation, but the system aims to minimize expert effort by making the \emph{code itself the trainable object} and iterating until convergence.

In summary, this paper makes three main contributions:
(1) We present \socia, a reliable, end-to-end simulator-code construction framework that requires minimal human supervision, coordinating heterogeneous LLM agents to synthesize, test, and refine executable simulators.
(2) We propose a \emph{textual computation graph} that embeds multi-agent reasoning and treats \emph{simulator code} as the \emph{optimization variable}, enabling \emph{loss-driven, constraint-aware textual-gradient updates} with momentum and projection.
(3) We demonstrate empirically that \socia constructs \emph{accurate, extrapolatable simulators} across CPS domains and across both aggregate and agent-based modeling granularities.


==> latex/chapter/2_related_old.tex <==
\textbf{Multi-agent systems (MAS) in Software Engineering.}
MAS are widely used for code and software generation~\cite{huang2023agentcoder,li2023camel,harper2024autogenesisagentselfgeneratingmultiagentsystems,jin2025llmsllmbasedagentssoftware}. Frameworks like MetaGPT~\cite{DBLP:conf/iclr/HongZCZCWZWYLZR24} and ChatDev~\cite{qian2024chatdev} formalize workflows via structured roles, while CodeR~\cite{chen2024coderissueresolvingmultiagent}, RGD~\cite{jin2024rgdmultillmbasedagent}, UnitTest~\cite{alshahwan2024automatedunittestimprovement}, and AI Scientist-v2~\cite{yamada2025ai} target specific phases (issue resolution, testing, or experimentation). 

\textbf{Simulator construction.}
Prior work spans: (1) \textbf{Domain-crafted simulators} which are authored by expert, creating an engineering bottleneck~\cite{zhang2025socioverse,DBLP:journals/corr/abs-2502-08691,DBLP:journals/corr/abs-2502-18712,jiawei2024large,yang2024oasis,tang2024gensim,yan2024opencity,law2007simulation};
(2) \textbf{LLM-based multi-agent systems} that compose simulators from natural-language scenarios but lack a closed, loss-aligned inner loop to edit code~\cite{DBLP:conf/ijcai/ChenDSZS00024,rasalLLMHarmonyMultiAgent2024,harper2024autogenesisagentselfgeneratingmultiagentsystems,shangAgentSquareAutomaticLLM2025,wang2025yulan,yue2025foam,cui2025talking};
(3) \textbf{Automated, data-calibrated pipelines} (e.g., G-Sim) that align models to observations yet emphasize aggregate calibration over localized code repair~\cite{DBLP:journals/corr/abs-2506-09272}.
\socia embeds specialized agents as nodes in a textual computation graph, enabling instance-level, constraint-aware code refinement.


\textbf{Textual gradients \& iterative self-improvement.}
DSPy~\cite{khattab2024dspy} formalizes LM pipelines as text-transformation graphs and optimizes them algorithmically; 
TextGrad~\cite{DBLP:journals/corr/abs-2406-07496} improves upstream components in compound systems by \emph{backpropagating textual feedback}; 
and Self-Refine~\cite{madaan2023self} and Reflexion~\cite{shinn2023reflexion} demonstrate that iterative critiques and episodic memory outperform one-shot prompting across tasks. 
Unlike generic textual-feedback methods, \socia performs simulator-specific credit assignment through a grounded blueprint: metric residuals are attributed to candidate mechanisms together with the spatial or interaction structures in which they operate before being converted into localized repair signals.



==> latex/chapter/3_approach_old.tex <==
%
As shown in Figure~\ref{fig:gradient}, the \socia framework addresses a central difficulty in automated simulator generation: generating runnable code is not sufficient, because the generated simulator may still implement the wrong behavioral mechanisms. 
A simulator can compile, execute, and produce outputs, yet fail to capture the intended agent states, interaction rules, intervention pathways, transition dynamics, or output-generation logic. 
Such mechanism-level errors are often not visible from code-level checks alone; instead, they appear as residuals between simulated outputs and observed aggregate behaviors.

\socia therefore treats simulator construction as a \emph{diagnosis-driven code optimization} problem. 
Given a task description and data, \socia first generates executable simulator code, runs the simulator, evaluates simulated outputs against observed behavioral signals, diagnoses which simulator mechanisms are likely responsible for the residual errors, and then produces localized code-repair feedback. 
This loop is organized as a \emph{textual computation graph}: agents exchange code, logs, metric values, residual summaries, diagnostic reports, and repair signals. 
Following TextGrad~\cite{DBLP:journals/corr/abs-2406-07496}, we retain the terminology of \emph{textual gradients}, \emph{Textual Gradient Descent}, \emph{optimizer}, \emph{momentum}, and \emph{projection}; however, in \socia these terms are used as operational abstractions for structured textual repair signals rather than numerical differentiation.

In this chapter, \S\ref{ssec:overview} introduces the diagnosis-driven optimization view; \S\ref{ssec:agent} describes the agents responsible for specification, execution, diagnosis, and repair; \S\ref{ssec:diagnosis} explains how aggregate metric residuals are linked to simulator mechanisms; and \S\ref{ssec:textgrad} formalizes the process using textual computation graphs, textual gradients, memory, and projection.
The detailed outer-loop algorithm is provided in Appendix~\ref{appen:detailed_workflow}.

\subsection{Diagnosis-Driven Simulator Code Optimization}
\label{ssec:overview}

The key challenge in simulator generation is not merely producing syntactically valid code, but producing code whose mechanisms match the target phenomenon. 
For example, a generated simulator may contain a plausible state-update function but use the wrong transition rule; it may include an intervention variable but connect it to the wrong agent behavior; or it may generate outputs in the correct schema while failing to reproduce the observed population-level dynamics. 
These failures are \emph{mechanism-level} rather than purely syntactic.

\socia closes this gap by converting behavioral residuals into mechanism-level repair signals. 
At iteration \(t\), the current simulator code \(x_t\) is executed on task inputs \(I\), producing simulator outputs \(o_t\). 
The outputs are compared against observed targets \(Y\) through task-specific metrics, producing aggregate losses and metric residuals. 
Rather than treating these residuals as scalar scores only, \socia uses them as diagnostic evidence: the system links each metric error to the simulator components that may have produced it, generates a mechanism-level diagnosis, and then translates the diagnosis into localized code-repair feedback.

This gives rise to an iterative loop:
\emph{code generation} $\rightarrow$ \emph{simulation execution} $\rightarrow$
\emph{residual evaluation} $\rightarrow$ \emph{mechanism diagnosis} $\rightarrow$
\emph{code repair} $\rightarrow$ \emph{constraint checking}.
The optimization target is therefore behavioral fidelity under executable-code constraints. 
The code itself remains the variable being optimized, but the update signal is not a numerical gradient. 
Instead, it is a structured textual gradient: a repair instruction grounded in metric residuals, execution evidence, and constraint violations.

\subsection{Orchestrated Agents}
\label{ssec:agent}

\paragraph{\textbf{Workflow Manager}}
The Workflow Manager controls the full optimization loop. 
It activates agents, passes artifacts along the textual computation graph, records iteration history, and terminates optimization when validation performance plateaus, the iteration budget is reached, or all required constraints hold. 
It also maintains the best feasible simulator encountered during optimization, allowing the system to fall back to a valid previous version if a later repair introduces failures.

\paragraph{\textbf{Data Analysis Agent (DAA)}}
DAA converts the task description, dataset, and task inputs into a structured simulator specification. 
Using a \texttt{data}-\texttt{schema}-\texttt{analysis} prompt, it identifies data fields, agent attributes, environmental variables, interaction relations, observable outputs, and links across data sources. 
Using a structured task-specification protocol, it then constructs the simulator brief by specifying: 
(1) target phenomena and modeling stance; 
(2) temporal resolution, spatial or interaction granularity, and population size; 
(3) agent units, static attributes, and dynamic states; 
(4) interaction mechanisms among agents or entities; 
(5) information-diffusion or influence pathways when applicable; 
(6) external signals or interventions and their access paths to simulator modules; 
(7) actions and decision policies; and 
(8) task-relevant metrics.

Crucially, DAA also constructs a \emph{grounded simulator blueprint} for later diagnosis. For each task metric, the blueprint records candidate simulator mechanisms that may affect that metric and, when supported by the task specification or data, the spatial or interaction context in which each mechanism operates. Such context may include spatial entities (e.g., POIs or anchors), spatiotemporal transitions, pairwise spatial relations, or typed interaction structures. This representation allows later feedback generation to distinguish not only which mechanism may explain a residual, but also the spatial or relational structure through which that mechanism affects simulator behavior.

\paragraph{\textbf{Code Generation Agent (CGA)}} 
CGA is responsible for both initial simulator synthesis and later code repair. 
It supports three working modes:
\begin{itemize}
    \item \emph{Initial code synthesis.} CGA reads the simulator specification and role description, then produces the initial runnable simulator code.
    \item \emph{Code optimization.} During iterative repair, CGA consumes textual gradients---i.e., structured mechanism-level repair feedback---and edits the simulator code accordingly.
    \item \emph{Constraint repair.} CGA applies minimal edits to satisfy hard constraints such as compilability, interface validity, I/O policy, deterministic execution, and output-schema conformity.
\end{itemize}
Additionally, CGA implements a self-check loop: after generating or editing code, it runs automatic checks for syntax errors, empty functions, interface mismatches, and runtime risks, and attempts local fixes for up to three rounds.

\paragraph{\textbf{Simulation Execution Agent (SEA)}} 
SEA compiles and executes the simulator code \(x_t\) on task inputs \(I\). 
It returns simulator outputs \(o_t\), intermediate traces when available, execution logs, timing information, and any compilation or runtime errors. 
These artifacts form the forward-pass evidence used by later evaluation and diagnosis.

\paragraph{\textbf{Result Evaluation Agent (REA)}} 
REA compares simulator outputs \(o_t\) with observed targets \(Y\) using task-specific metrics. 
Its role is not limited to reporting scalar losses. 
It decomposes evaluation results into metric residuals, identifies abnormal output patterns, and records constraint violations. 
In this way, REA converts raw simulator behavior into structured diagnostic evidence that can be consumed by the feedback agent.

\paragraph{\textbf{Feedback Generation Agent (FGA)}} 
FGA converts residual evidence into mechanism-grounded repair feedback. Given the current simulator, metric residuals, execution evidence, constraint violations, and the grounded blueprint produced by DAA, FGA performs residual-to-mechanism attribution. For spatially grounded mechanisms, this attribution explicitly conditions on their associated spatial entities, transitions, relations, or interaction structures. The resulting diagnosis identifies a likely faulty mechanism together with the context in which its mismatch manifests. FGA then converts this diagnosis into a textual gradient: a localized repair signal specifying what simulator mechanism should be revised and why.

With these agents, \socia separates the simulator-generation process into specification, execution, evaluation, diagnosis, repair, and constraint checking. 
This decomposition is important because aggregate losses alone rarely indicate how simulator code should be changed; the agents provide the intermediate reasoning steps required to turn loss into executable repair.

\subsection{From Behavioral Residuals to Grounded Mechanism Diagnosis}
\label{ssec:diagnosis}

The central operation in \socia is the conversion:
\[
\text{metric residual}
\;\rightarrow\;
\text{mechanism diagnosis}
\;\rightarrow\;
\text{code repair feedback}.
\]
This operation is task-general. 
The specific metrics differ across domains, but the diagnostic procedure is the same: metric errors are linked to the simulator blueprint, the likely faulty mechanisms are identified, and localized repair instructions are generated for the code agent.

\paragraph{\textbf{Metric Residual Construction}}
Given simulator output \(o_t\) and observed targets \(Y\), REA computes a set of task-specific metrics:
\[
\mathbf{m}_t = [m_t^{(1)}, m_t^{(2)}, \ldots, m_t^{(K)}],
\]
where each metric measures one observable dimension of simulator fidelity. 
The metric residual vector is then:
\[
\mathbf{r}_t = \mathrm{Residual}(\mathbf{m}_t, \mathbf{m}^{\star}),
\]
where \(\mathbf{m}^{\star}\) denotes the target or reference metric values derived from observations. 
A scalar validation loss \(L_t\) may be computed by aggregating these residuals, but \socia preserves the individual residual components because different metrics point to different simulator mechanisms.

% \paragraph{\textbf{Residual-to-Mechanism Linking}}
% The simulator blueprint produced by DAA stores a mapping between metrics and candidate simulator components:
% \[
% \mathcal{B}: m^{(k)} \mapsto \{h_1, h_2, \ldots, h_q\},
% \]
% where each \(h\) denotes a possible mechanism or code region, such as an agent state variable, interaction function, transition rule, intervention handler, calibration parameter, or output-construction routine. 
% This mapping does not mechanically determine the repair. 
% Instead, it restricts diagnosis to plausible simulator mechanisms and prevents the feedback process from issuing generic, ungrounded suggestions.

\textbf{Grounded Residual-to-Mechanism Linking.}
The simulator blueprint produced by DAA associates each evaluation
metric with candidate simulator mechanisms and, when applicable,
their spatial or interaction grounding:
\begin{equation}
\mathcal{B}:m^{(k)}
\mapsto
\left\{(h_j,\rho_j)\right\}_{j=1}^{q},
\end{equation}
where $h_j$ denotes a candidate simulator mechanism or code component,
such as an agent state variable, interaction function, transition rule,
intervention handler, calibration parameter, or output-construction
routine. The grounding variable $\rho_j$ represents the spatial or
interaction structure through which $h_j$ affects the observable,
including spatial entities, spatiotemporal transitions, spatial relations,
anchors, or typed interaction layers.

The grounding is evidence-bounded: when no spatial or interaction
structure is supported by the task or data, $\rho_j$ is left unspecified.
Thus, $\rho_j$ should not be interpreted as a geographic error location
or a hard spatial constraint. Instead, it provides structured context for
credit assignment, restricting diagnosis to mechanisms and relational
structures that are plausible explanations of the observed residual.

\paragraph{\textbf{Mechanism Diagnosis and Repair Feedback}}
% FGA combines the residual vector, the blueprint mapping, execution logs, constraint violations, and the current code to produce a diagnosis:
% \[
% d_t = \mathcal{D}_{\mathrm{LLM}}(x_t, \mathbf{r}_t, \mathcal{B}, e_t, v_t),
% \]
% where \(e_t\) denotes execution evidence and \(v_t\) denotes constraint violations. 
% The diagnosis \(d_t\) identifies likely simulator failure modes and affected components. 
% FGA then converts this diagnosis into a textual gradient:
% \[
% g_t = \mathcal{G}_{\mathrm{LLM}}(x_t, d_t, \mathbf{r}_t, e_t, v_t),
% \]
% where \(g_t\) is a structured repair signal specifying how the simulator code should change. 
% Thus, the textual gradient is not merely a free-form critique; it is a mechanism-grounded instruction derived from observed residuals and routed toward code repair.
%
FGA combines the residual vector, grounded blueprint, current simulator,
execution evidence, and constraint violations to produce
\begin{equation}
d_t =
D_{\mathrm{LLM}}
(x_t,r_t,\mathcal{B},e_t,v_t).
\end{equation}

Conceptually, the diagnosis performs the attribution
\begin{equation}
(r_t,\mathcal{B})
\;\longrightarrow\;
(\hat h_t,\hat\rho_t),
\end{equation}
where $\hat h_t$ denotes a likely mechanism associated with the residual
and $\hat\rho_t$ denotes the relevant spatial or interaction context.
The pair $(\hat h_t,\hat\rho_t)$ is a diagnostic attribution rather than
a causal guarantee: execution evidence and residual patterns may support
multiple plausible mechanisms.

% \subsection{Textual-Gradient Optimization}
% \label{ssec:textgrad}

% Following TextGrad~\cite{DBLP:journals/corr/abs-2406-07496}, we abstract the \socia pipeline as a textual computation graph. 
% This abstraction allows us to express simulator-code repair using familiar optimization terminology while keeping the implementation grounded in concrete diagnostic and repair operations.

% \paragraph{\textbf{(1) Problem Definition}}
% We study instance optimization of a simulator whose implementation is itself the trainable object.
% \begin{itemize}
%   \item \textbf{Task brief:} \(D\), generated by DAA through structured data and task analysis.
%   \item \textbf{Data:} task inputs \(I\) and observed targets \(Y\).
%   \item \textbf{Variable:} \(x \in \mathcal{X}\), a runnable simulator program represented as code.
%   \item \textbf{Role description:} \(r\), specifying the simulator's intended interface, I/O behavior, semantics, and constraints.
%   \item \textbf{Hard constraints:}
%   \[
%   \mathcal{C} = \{x : c_j(x) \le 0,\; j=1,\ldots,J\}.
%   \]
%   These constraints include no syntax errors, compilability, valid file access, non-empty execution flow, deterministic behavior when required, and output-schema conformity.
%   \item \textbf{Optimization goal:}
%   \[
%   \min_{x \in \mathcal{X}} L(x)
%   \quad
%   \text{s.t.}
%   \quad
%   x \in \mathcal{C}.
%   \]
%   Here \(L(x)\) measures behavioral mismatch between simulated and observed outputs, while \(\mathcal{C}\) ensures that the resulting simulator remains executable and valid.
% \end{itemize}
% We use \(LLM(z)\) to denote prompting a language model with input \(z\) and collecting its response.

% \paragraph{\textbf{(2) Textual Computation Graph}}
% We model the system as a DAG \(\mathcal{G}=(V,E)\). 
% Nodes are black-box operators: LLM nodes generate or edit text, while function nodes execute code, compute metrics, check constraints, or aggregate logs. 
% Edges carry artifacts such as simulator code, task specifications, execution outputs, metric residuals, diagnostic reports, and repair feedback.

% Each node \(v\) computes:
% \[
% z_v = f_v(\{z_u : u \in \mathrm{Pa}(v)\}),
% \]
% where \(\mathrm{Pa}(v)\) denotes the parents of node \(v\). 
% Many \(f_v\) are non-differentiable, including LLM calls, compilers, and simulators. 
% We therefore use textual gradients to enable backward signal flow: downstream behavioral residuals are converted into natural-language repair signals for upstream textual variables, especially simulator code.

% \paragraph{\textbf{(3) Forward Pass and Loss with Constraints}}
% Code initialization produces the first simulator:
% \[
% x_0 = f_{\mathrm{LLM}}(D, r).
% \]
% At iteration \(t\), SEA executes the current simulator:
% \[
% o_t = f_{\mathrm{Sim}}(x_t, I),
% \]
% where \(o_t\) includes simulated observables and, when available, execution traces. 
% REA then computes:
% \[
% L_t = \ell(o_t, Y) + \lambda \sum_j \max(0, c_j(x_t)).
% \]
% The first term measures behavioral mismatch; the second term penalizes constraint violations. 
% In addition to this scalar objective, REA also outputs the metric residual vector \(\mathbf{r}_t\), execution evidence \(e_t\), and constraint-violation report \(v_t\), which are used for diagnosis.

% \paragraph{\textbf{(4) Textual Gradients: Backward Signal as Repair}}
% Following the TextGrad notation, we write the backward signal as a textual gradient with respect to the code variable:
% \[
% g_t \triangleq \frac{\partial L_t}{\partial x_t}.
% \]
% Since \(x_t\) is simulator code and the execution pipeline contains non-differentiable components, \(\frac{\partial L_t}{\partial x_t}\) is not a numerical derivative. 
% Rather, it denotes a structured repair signal that explains how \(x_t\) should be changed to reduce \(L_t\). 
% The notation is useful because it captures responsibility routing in the computation graph: downstream metric residuals are propagated backward to upstream textual variables.

% In analogy to the chain rule, we write:
% \[
% \frac{\partial L_t}{\partial x_t}
% =
% \frac{\partial L_t}{\partial o_t}
% \cdot
% \frac{\partial o_t}{\partial x_t}
% \;\rightsquigarrow\;
% \nabla_{\mathrm{LLM}}(x_t, o_t, \mathbf{r}_t, d_t, e_t, v_t).
% \]
% Here, \(\frac{\partial L_t}{\partial o_t}\) is operationalized as metric residuals and output criticisms, while \(\frac{\partial o_t}{\partial x_t}\) is operationalized as mechanism attribution over the simulator code. 
% The resulting textual gradient is:
% \[
% g_t =
% \nabla_{\mathrm{LLM}}(x_t, o_t, \mathbf{r}_t, d_t, e_t, v_t),
% \]
% where \(d_t\) is the mechanism diagnosis produced by FGA. 
% Operationally, \(g_t\) is a set of localized, actionable code-edit instructions rather than a numeric gradient vector.

% \paragraph{\textbf{(5) Textual Momentum as History-Aware Repair Memory}}
% To stabilize long-horizon editing, \socia maintains a textual momentum buffer. 
% Following the terminology of momentum in optimization, we define:
% \[
% m_t = \mathrm{Decay}_{\beta}(m_{t-1}) \oplus g_t,
% \]
% where \(\oplus\) denotes ordered merge and \(\mathrm{Decay}_{\beta}\) down-weights stale items. 
% In implementation, \(m_t\) is a concise textual memory over recent diagnoses, failed repairs, successful fixes, and unresolved issues. 
% We keep the latest \(K\) iterations, with \(K=3\) in our experiments.

% This memory prevents repeated mistakes and reduces oscillatory edits. 
% Rather than asking CGA to respond only to the current residual, \socia provides the optimizer with recent repair context: what failed before, what was already fixed, and which simulator components should not be disturbed. 
% Thus, textual momentum acts as history-aware repair memory while retaining the optimization analogy.

% \paragraph{\textbf{(6) Textual Gradient Descent and Projected Gradient Descent}}
% Given the aggregated textual gradient \(m_t\), the optimizer performs a Textual Gradient Descent step:
% \[
% x_{t+1}^{\mathrm{unproj}}
% =
% \mathrm{TGD.step}(x_t, m_t; r).
% \]
% Operationally, \(\mathrm{TGD.step}\) is implemented by CGA as a code-repair operator. 
% It edits simulator mechanisms according to the textual gradient while preserving unaffected components whenever possible. 
% The output \(x_{t+1}^{\mathrm{unproj}}\) is the repaired but not-yet-validated simulator code.

% Analogous to Projected Gradient Descent (PGD), \socia then applies a textual projection step that maps the raw edited code back to the feasible set:
% \[
% x_{t+1}
% =
% \Pi_{\mathcal{C}}(x_{t+1}^{\mathrm{unproj}}),
% \qquad
% \Pi_{\mathcal{C}}: \mathcal{T} \rightarrow \{x : c_j(x)\le 0\ \forall j\}.
% \]
% The projector performs static checks, interface tests, compilation checks, schema validation, and other task-specific feasibility checks. 
% If a violation is detected, CGA performs minimal-edit repair through the \texttt{code}-\texttt{fix} prompt and repeats the self-check loop for up to three attempts. 
% The projection step therefore ensures that behavioral repair does not sacrifice executability or interface validity.

% \paragraph{\textbf{(7) One-Line Summary (All Pieces Together)}}

% \begin{simstepbox}
% \begin{tabularx}{\linewidth}{@{}l X@{}}

% \textbf{Forward:} &
% \(
% \begin{aligned}[t]
% o_t &= f_{\mathrm{Sim}}(x_t, I),\\
% L_t &= \ell(o_t, Y) + \lambda \sum_j \max(0, c_j(x_t)).
% \end{aligned}
% \)\\[4pt]

% \textbf{Diagnosis:} &
% \(
% \begin{aligned}[t]
% \mathbf{r}_t &= \mathrm{Residual}(\mathbf{m}_t, \mathbf{m}^{\star}),\\
% d_t &= \mathcal{D}_{\mathrm{LLM}}(x_t, \mathbf{r}_t, \mathcal{B}, e_t, v_t).
% \end{aligned}
% \)\\[4pt]

% \textbf{Backward:} &
% \(
% g_t = \frac{\partial L_t}{\partial x_t}
% \rightsquigarrow
% \nabla_{\mathrm{LLM}}(x_t, o_t, \mathbf{r}_t, d_t, e_t, v_t)
% \)\\[4pt]

% \textbf{Momentum:} &
% \(m_t = \mathrm{Decay}_{\beta}(m_{t-1}) \oplus g_t\)\\[4pt]

% \textbf{Update:} &
% \(
% \begin{aligned}[t]
% x_{t+1}^{\mathrm{unproj}} &= \mathrm{TGD.step}(x_t, m_t; r),\\
% x_{t+1} &= \Pi_{\mathcal{C}}(x_{t+1}^{\mathrm{unproj}}).
% \end{aligned}
% \)\\
% \end{tabularx}
% \end{simstepbox}

% We iteratively optimize \(x\) and stop when validation loss plateaus and all hard constraints hold, or when the iteration budget is reached. 
% If a later update violates constraints, the Workflow Manager can return the best feasible simulator from previous iterations.

% \paragraph{\textbf{What the Textual Gradient Encodes}}
% The textual gradient in \socia is not merely a free-form critique. 
% It encodes three linked operations:
% \begin{itemize}
%     \item \textbf{Residual-to-diagnosis:} aggregate behavioral residuals are converted into interpretable simulator failure modes by linking metric errors to the simulator blueprint and candidate code mechanisms.
%     \item \textbf{Diagnosis-to-repair feedback:} diagnosed failure modes are translated into localized code-edit instructions, specifying which mechanism should be added, removed, or revised.
%     \item \textbf{Repair-to-executable simulator:} CGA applies the repair feedback to simulator code, while the projection step enforces compilability, interface validity, output-schema conformity, and other hard constraints.
% \end{itemize}


\subsection{Textual-Gradient Repair Abstraction}
\label{ssec:textgrad}

Following TextGrad~\cite{DBLP:journals/corr/abs-2406-07496}, we
represent the \socia pipeline as a textual computation graph and use
gradient-inspired terminology to organize backward credit assignment and
iterative repair. These terms are operational abstractions rather than
numerical differentiation: we do not assume differentiability of the
simulator pipeline or monotonic improvement of the resulting updates.

\paragraph{\textbf{(1) Problem Definition}}
We study iterative refinement of an executable simulator program.
\begin{itemize}
    \item \textbf{Task brief:} \(D\), generated by DAA through
    structured data and task analysis.
    
    \item \textbf{Data:} task inputs \(I\) and observed targets \(Y\).
    
    \item \textbf{Variable:} \(x \in \mathcal{X}\), a runnable
    simulator program represented as code.
    
    \item \textbf{Role description:} \(r\), specifying the simulator's
    intended interface, I/O behavior, semantics, and constraints.
    
    \item \textbf{Hard constraints:}
    \[
    \mathcal{C}
    =
    \{x:c_j(x)\leq0,\;j=1,\ldots,J\}.
    \]
    These constraints include syntactic validity, compilability,
    valid file access, non-empty execution flow, deterministic behavior
    when required, and output-schema conformity.
    
    \item \textbf{Refinement objective:}
    \[
    \min_{x\in\mathcal{X}} L(x)
    \qquad
    \text{s.t.}\qquad
    x\in\mathcal{C}.
    \]
    Here \(L(x)\) measures behavioral mismatch between simulated and
    observed outputs, while \(\mathcal{C}\) ensures that the simulator
    remains executable and valid.
\end{itemize}
We use \(LLM(z)\) to denote prompting a language model with input \(z\)
and collecting its response.

\paragraph{\textbf{(2) Textual Computation Graph}}
We model the system as a DAG \(\mathcal{G}=(V,E)\).
Nodes are black-box operators: LLM nodes generate or edit textual
artifacts, while function nodes execute code, compute metrics, check
constraints, or aggregate evidence. Edges carry simulator code, task
specifications, execution outputs, metric residuals, grounded diagnoses,
and repair feedback.

Each node \(v\) computes
\[
z_v=f_v(\{z_u:u\in\mathrm{Pa}(v)\}),
\]
where \(\mathrm{Pa}(v)\) denotes the parents of \(v\).
Many \(f_v\) are non-differentiable, including LLM calls, compilers,
and simulators. We therefore use textual gradients as structured backward
signals: downstream behavioral residuals are attributed to upstream
simulator mechanisms and converted into localized repair instructions.

\paragraph{\textbf{(3) Forward Pass and Behavioral Residuals}}
Code initialization produces the first simulator:
\[
x_0=f_{\mathrm{LLM}}(D,r).
\]
At iteration \(t\), SEA executes the current simulator:
\[
o_t=f_{\mathrm{Sim}}(x_t,I),
\]
where \(o_t\) contains simulated observables and, when available,
execution traces. REA computes
\[
L_t
=
\ell(o_t,Y)
+
\lambda\sum_j\max(0,c_j(x_t)).
\]
The first term measures behavioral mismatch and the second penalizes
constraint violations. Importantly, REA also preserves the metric residual
vector \(\mathbf r_t\), together with execution evidence \(e_t\) and
constraint violations \(v_t\), rather than reducing all evaluation
information to the scalar \(L_t\).

\paragraph{\textbf{(4) Textual Gradient as Grounded Credit Assignment}}
The backward repair signal is represented as a textual gradient
\[
g_t
=
\mathcal{G}_{\mathrm{LLM}}
(x_t,\mathbf r_t,d_t,e_t,v_t),
\]
where \(d_t\) is the grounded mechanism diagnosis defined in
\S\ref{ssec:diagnosis}. Operationally, this backward process performs
two levels of credit assignment. First, the metric residuals
\(\mathbf r_t\) identify which observable dimensions of simulator
behavior are mismatched. Second, the grounded blueprint
\(\mathcal B\) attributes these mismatches to candidate simulator
mechanisms and, when applicable, to the spatial or interaction structures
through which those mechanisms operate:
\[
(\mathbf r_t,\mathcal B)
\longrightarrow
(\hat h_t,\hat\rho_t)
\longrightarrow
d_t
\longrightarrow
g_t.
\]
Here \(\hat h_t\) denotes a likely residual-relevant simulator mechanism
and \(\hat\rho_t\) its associated spatial or interaction context.
Consequently, \(g_t\) is not a numerical gradient vector or a generic
critique; it is a localized repair direction conditioned on the grounded
diagnosis. It specifies how the diagnosed mechanism should be revised
while preserving unrelated mechanisms and spatial or interaction
structures whenever possible.

\paragraph{\textbf{(5) Textual Momentum as History-Aware Repair Memory}}
To stabilize long-horizon editing, \socia maintains a textual momentum
buffer:
\[
m_t
=
\mathrm{Decay}_{\beta}(m_{t-1})
\oplus
g_t,
\]
where \(\oplus\) denotes ordered merge and
\(\mathrm{Decay}_{\beta}\) down-weights stale items.
In implementation, \(m_t\) is a concise textual memory over recent
diagnoses, failed repairs, successful fixes, and unresolved issues.
We retain the latest \(K\) iterations, with \(K=3\) in our experiments.

Rather than responding only to the current residual, CGA therefore
receives recent repair context describing what failed previously, what
has already been repaired, and which simulator mechanisms should remain
unchanged. Textual momentum thus serves as history-aware repair memory
within the gradient-inspired abstraction.

\paragraph{\textbf{(6) Textual Repair and Constraint Projection}}
Given the aggregated textual repair signal \(m_t\), CGA performs the
TGD-style update
\[
x_{t+1}^{\mathrm{unproj}}
=
\mathrm{TGD.step}(x_t,m_t;r),
\]
where \(\mathrm{TGD.step}\) denotes an LLM-based code-repair operator
rather than numerical gradient descent. It applies the grounded repair
signal to the diagnosed simulator mechanism while preserving unaffected
components whenever possible.

A subsequent projection-style repair maps the edited simulator back to
the feasible set:
\[
x_{t+1}
=
\Pi_{\mathcal C}
(x_{t+1}^{\mathrm{unproj}}),
\qquad
\Pi_{\mathcal C}:
\mathcal T
\rightarrow
\{x:c_j(x)\leq0\ \forall j\}.
\]
The projector performs static checks, interface tests, compilation checks,
schema validation, and other task-specific feasibility checks. If a
violation is detected, CGA performs minimal-edit repair and repeats the
self-check procedure. The projection step therefore preserves executable
and interface constraints; it should not be interpreted as imposing
additional geographic or spatial feasibility constraints.

\paragraph{\textbf{(7) One-Line Summary}}
The complete refinement pathway is:
\begin{simstepbox}
\begin{tabularx}{\linewidth}{@{}l X@{}}

\textbf{Forward:} &
\(
\begin{aligned}[t]
o_t &= f_{\mathrm{Sim}}(x_t,I),\\
L_t &= \ell(o_t,Y)
      +\lambda\sum_j\max(0,c_j(x_t)).
\end{aligned}
\)
\\[4pt]

\textbf{Residual:} &
\(
\mathbf r_t
=
\mathrm{Residual}
(\mathbf m_t,\mathbf m^{\star})
\)
\\[4pt]

\textbf{Grounding:} &
\(
(\mathbf r_t,\mathcal B)
\rightarrow
(\hat h_t,\hat\rho_t)
\rightarrow
d_t
\)
\\[4pt]

\textbf{Backward:} &
\(
g_t
=
\mathcal{G}_{\mathrm{LLM}}
(x_t,\mathbf r_t,d_t,e_t,v_t)
\)
\\[4pt]

\textbf{Momentum:} &
\(
m_t
=
\mathrm{Decay}_{\beta}(m_{t-1})
\oplus g_t
\)
\\[4pt]

\textbf{Update:} &
\(
\begin{aligned}[t]
x_{t+1}^{\mathrm{unproj}}
&=
\mathrm{TGD.step}(x_t,m_t;r),\\
x_{t+1}
&=
\Pi_{\mathcal C}
(x_{t+1}^{\mathrm{unproj}}).
\end{aligned}
\)
\\

\end{tabularx}
\end{simstepbox}

The system stops when validation performance plateaus and the required
hard constraints hold, or when the outer-loop budget is reached. If a
later repair violates feasibility constraints, the Workflow Manager can
return the best feasible simulator observed in earlier iterations.

\paragraph{\textbf{What the Textual Gradient Encodes}}
The textual gradient in \socia represents three linked operations:
\begin{itemize}
    \item \textbf{Residual-to-grounded diagnosis:}
    behavioral residuals are attributed to candidate simulator mechanisms
    together with their relevant spatial or interaction contexts.

    \item \textbf{Diagnosis-to-localized repair:}
    the diagnosed mechanism and grounding context are translated into
    targeted repair instructions while unrelated simulator mechanisms are
    preserved whenever possible.

    \item \textbf{Repair-to-feasible simulator:}
    CGA applies the repair signal to executable simulator code, while
    projection preserves compilability, interface validity,
    output-schema conformity, and other hard execution constraints.
\end{itemize}

==> latex/chapter/3_approach_old_old.tex <==
%
As shown in Figure~\ref{fig:gradient}, the \socia framework adopts a multi-agent architecture tailored to constructing high-fidelity simulators across heterogeneous CPS domains. 
Given a task description and data as inputs, \socia outputs \emph{runnable, high-quality simulator code}; once executed by the user, this code launches a high-fidelity simulator.
%
In this chapter, \S\ref{ssec:computation_graph} elaborates the notions of \textbf{computation graphs} and \textbf{textual gradients}; \S\ref{ssec:agent} describes the roles and capabilities of different \textbf{agents} in \socia; and \S\ref{ssec:textgrad} explains how these agent functions are embedded into the computation graph and how \textbf{textual-gradient computation and backpropagation} are used to optimize the simulator code.

\subsection{Computation Graphs and Textual Gradients}
\label{ssec:computation_graph}

In mainstream ML, a computation graph is a directed acyclic graph (DAG) whose nodes are operations and whose edges carry intermediate values~\cite{bergstra2010theano,jia2014caffe,abadi2016tensorflow,paszke2019pytorch}; the forward pass evaluates the graph, and the backward pass applies the chain rule to accumulate gradients for parameter updates~\cite{amari1993backpropagation}.

Nowadays, many researchers have begun \emph{building compound AI systems with LLMs}, abstracting complex AI pipelines as \emph{textual computation graphs} and using \emph{differentiation and gradients as a metaphor for LLM-produced textual feedback}~\cite{shinn2023reflexion,pryzant2023automatic,DBLP:journals/corr/abs-2406-07496}. This leverages LLMs’ strengths in \emph{reasoning, self-checking, and self-refinement}~\cite{bai2022training,madaan2023self,shinn2023reflexion,li2023alpacaeval,khattab2024dspy,yuan2024self} to optimize AI systems.

In \socia, we lift this idea from numeric operators to an \emph{agentic pipeline} that builds a high-fidelity simulator. Each agent that performs a specific function or behavior is a \textbf{node} in the DAG; \textbf{edges} pass text or numeric artifacts (code, logs, metrics). Many nodes are \emph{non-differentiable} (e.g., LLM calls, compilers, simulators). Following TextGrad~\cite{DBLP:journals/corr/abs-2406-07496}, we endow this computation graph with \textbf{textual gradients}—natural-language critiques that describe how to modify upstream textual variables (here, the simulator code) to improve the downstream objective (high-fidelity simulation). The framework explicitly mirrors the \emph{autograd} metaphor but with \emph{text as the gradient carrier}, and provides a \emph{PyTorch-like paradigm}~\cite{paszke2019pytorch} to define losses and update variables.

As a textual-gradient paradigm with a prompt-LLM backbone, we must ask: \textbf{why textual gradients over plain prompt engineering?} 
Prompt engineering is model/version-dependent, phrasing-sensitive, and hard to evaluate systematically~\cite{salinas2024butterfly}, yielding brittleness, poor portability, and dependence on measurement protocols~\cite{polo2024efficient}. 
\emph{Textual gradients} recast the problem as \emph{principled optimization}—a \emph{loss-driven, backprop-style loop} over the whole system that produces targeted, evidence-grounded updates and improves reproducibility and comparability~\cite{khattab2024dspy}. 
Rather than global prompt fiddling, textual gradients enable \emph{local, loss-aligned edits}: downstream signals (metric diffs, failing cases, constraint violations) are turned into \emph{machine-readable, executable feedback} and routed to the responsible node (e.g., a faulty function), after which an optimizer LLM proposes \emph{small, verifiable} patches that preserve working components. 
Moreover, \emph{iterative, feedback-driven refinement} consistently outperforms one-shot prompting~\cite{madaan2023self,shinn2023reflexion}, reinforcing the superiority of \emph{loss-aligned local edits} over \emph{global prompt tweaks}. 
\emph{In sum}, textual gradients transform brittle, template-tuned systems into \emph{reliable, loss-aligned optimization pipelines} with \emph{targeted, verifiable updates} that scale across agents and tasks—precisely what plain prompt engineering struggles to offer.


\subsection{Orchestrated Agents}
\label{ssec:agent}
\paragraph{\textbf{Workflow Manager}}
Serving as the hub, the Workflow Manager controls the multi-agent workflow. Following the computation-graph design, it activates different agents, loads the task-specific prompts that instruct each agent, executes the graph’s forward/backward computations in order, and terminates the iteration according to the convergence status of code optimization.

\paragraph{\textbf{Code Generation Agent (CGA)}} CGA supports multiple prompts that each is aligned with a distinct function. It ships with three working prompts: 
\begin{itemize}
    \item \emph{Initial code synthesis.} Before gradient computation begins, CGA reads the task brief and the predefined role description (see \S\ref{ssec:textgrad}) and, using the \texttt{code}-\texttt{generation} prompt, produces the initial simulator code.
    \item \emph{Code optimization.} During textual-gradient–based optimization, CGA loads the \texttt{code}-\texttt{optimization} prompt and upgrades the code according to the back-propagated textual gradients (i.e., critiques on how to improve the code).
    \item \emph{Constraint repair.} CGA loads the \texttt{code}-\texttt{fix} prompt to handle \emph{hard constraints}—coding conventions, interface contracts, and I/O requirements for the simulator (see \S\ref{ssec:textgrad}).
\end{itemize}

Additionally, CGA implements a \textbf{self-loop} mechanism: after generating/optimizing code, it performs automatic quality checks (e.g., compilation, syntax/static analyses for potential runtime errors, empty-function checks), aggregates all detected issues, and applies improvements. This \emph{self-check $\rightarrow$ fix} cycle runs up to three times per iteration to enhance robustness.

\paragraph{\textbf{Simulation Execution Agent (SEA)}} 
The SEA compiles and executes the simulator code, generates simulation outputs (e.g., agent trajectories or actions), and records any compilation or runtime errors encountered during execution.

\paragraph{\textbf{Result Evaluation Agent (REA)}} 
Given SEA’s predictions and error logs, the REA computes fidelity losses using task-specific evaluation metrics and performs code diagnostics based on the compilation and runtime errors reported by SEA. The REA incorporates \emph{constraint satisfaction} into the overall loss computation.

\paragraph{\textbf{Feedback Generation Agent (FGA)}} 
FGA provides two dedicated working prompts. When \emph{REA}’s computed losses and diagnostic reports are available, the FGA loads the \texttt{output}-\texttt{criticism} prompt to analyze the comparison between the simulator’s outputs and the ground truth for the current iteration—identifying where the output falls short, whether predictions exhibit distortion, and under what conditions such distortion arises.
In parallel, the FGA maintains a \textbf{historic log} that records past errors and their corresponding fixes. Conditioned on the current simulation code and the output criticisms, the FGA loads the \texttt{gradient}-\texttt{generation} prompt and performs both prediction attribution analysis (highlighting failure modes or undesirable behaviors) and code-correction analysis, proposing \emph{executable, code-improving patches} to remedy detected issues. It also summarizes recent errors and fixes from the history window and integrates them with the current round’s code-edit proposals before delivering them to the CGA.

\paragraph{\textbf{Data Analysis Agent (DAA)}}
DAA first consolidates the task description, the task dataset, and task inputs (e.g., agent-related data such as profiles, historical trajectories, and community context). Using a \texttt{data}-\texttt{schema}-\texttt{analysis} prompt, it infers the \textbf{data schema}: attribute analyses, linkage and interaction relationships across data sources, and the connections between these data and simulator construction (e.g., which data build agent profiles vs. which define the environment). Next, DAA loads a \texttt{task}-\texttt{brief}-\texttt{analysis} prompt and, guided by a chain-of-thought (\textbf{CoT}) procedure~\cite{wei2022chain}, iteratively reasons through and answers the following to produce the simulator’s \textbf{task brief}: (1) clarify target phenomena/outcomes and modeling stance; (2) specify time step, spatial resolution, and population size; (3) define agent unit(s) and roles; list static attributes and dynamic states of agents; (4) describe agent interactions; (5) determine whether/how information diffuses; (6) identify external signals/interventions and their access paths to agents/modules; (7) define actions and the policy mapping observations/signals to actions; (8) define task-relevant metrics.

Importantly, \emph{after} DAA drafts the task brief, we introduce a \textbf{human-in-the-loop (HITL)} stage~\cite{so2020human,wu2022survey,mosqueira2023human,natarajan2025human}: domain experts review and provide feedback to confirm the simulator design. DAA incorporates human feedback, produces a revised task brief, and repeats expert confirmation until approval. In practice, leaving all design choices solely to an LLM can lead to \emph{hallucinations}~\cite{liu2024exploring,xu2024hallucination}; due to CoT, early hallucinations may \emph{propagate} through the reasoning process, causing substantial \emph{semantic drift} between the LLM’s final design and user intent~\cite{xue2023rcot,yee2024faithful}. Incorporating expert feedback corrects such drift and significantly mitigates these issues~\cite{amirizaniani2024developing,tonmoy2024comprehensive}. The goal is to combine the LLM’s efficiency with human judgment to improve system reliability and safety.

With these definitions of the central manager and agents in \socia, the agents are instantiated as nodes in the computation graph described in \S\ref{ssec:textgrad}.


\subsection{Textual-Gradient Optimization}
\label{ssec:textgrad}

Following \emph{TextGrad}~\cite{DBLP:journals/corr/abs-2406-07496}, we abstract our AI system as a \textbf{computation graph}, where functionally distinct agents are represented as graph nodes. 
Optimizing the simulator code becomes an \emph{instance optimization problem}: we treat the code itself as an \textbf{optimization variable}, compute ``\emph{textual gradients}'' for that variable via a backpropagation-like mechanism, and then apply a gradient-descent-style procedure to iteratively improve the \emph{code variable}.

\paragraph{\textbf{(1) Problem Definition}}
We study \emph{instance optimization} of a simulator whose implementation is itself the trainable object. 
\begin{itemize}
  \item \textbf{Task brief (natural language):} \(D\) (generated by the \textbf{DAA} after executing the \texttt{task}-\texttt{brief}-\texttt{analysis} prompt).
  \item \textbf{Data:} task inputs \(I\) and ground-truth observables \(Y\).
  \item \textbf{Variable:} \(x \in \mathcal{X}\), which is a \emph{runnable simulator program} (code string).
  \item \textbf{Role description (text):} \(r\), specifies the intended interface/IO/semantics of \(x\).
  \item \textbf{Hard constraints (feasible set):}
$\mathcal{C}=\{\,x:\; c_j(x)\le 0,\ j=1,\dots,J\,\}$. 
Here, \emph{constraints} constitute an important part of our design, serving to restrict the generated simulator code so that it adheres to domain-specific requirements or predefined specifications. They are design rules for the simulator code, such as: \emph{no syntax errors; compilable; read files according to policy; non-empty main flow; outputs match the specified schema}, etc.
  \item \textbf{Inequality-constrained Optimization Goal:} 
  \[
  \min_{x\in \mathcal{X}} L(x)\ \ \text{s.t.}\ \ x\in \mathcal{C}
  \] 
  Our objective is to ensure that, under the constraints $\mathcal{C}$, the generated code $x$ achieves minimum fidelity-loss.
  \item We use the notation \textbf{$LLM(z)$} to denote giving $z$ as a prompt to a language model and collecting its response.
\end{itemize}

\paragraph{\textbf{(2) Textual Computation Graph}}
We model the system as a DAG \(\mathcal{G}=(V,E)\), whose nodes are \emph{black-box operators}:
\begin{itemize}
  \item \emph{LLM nodes} produce or edit text (e.g., code).
  \item \emph{Function nodes} execute code or compute metrics.
  % \item \emph{Combiners} merge multiple signals.
\end{itemize}

Each node \(v\) computes $ z_v = f_v(\{z_u : u \in \mathrm{Pa}(v)\})$, 
where \(f_v\) is a function that performs a specific capability, and \(\mathrm{Pa}(v)\) denotes the parents of node \(v\). 
In our setting, all nodes correspond to \textbf{agents} in \socia with different abilities. 
Although \(f_v\) may be \emph{non-differentiable}, we enable \emph{backward signal flow} via \emph{textual gradients}---natural-language critiques that explain how to change an upstream text variable to reduce downstream loss.

\paragraph{\textbf{(3) Forward Pass and Loss with Constraints}}

We first perform \emph{code initialization} by synthesizing the code variable: $ x_0 = f_{\mathrm{LLM}}(D, r) $,
where the \emph{input} is the task description \(D\) (natural-language brief) and the role description \(r\) (the required interface/constraints for the simulator code). The \emph{output} is the initial simulator program \(x_0\) as text (simulator code). The \emph{job} of this mapping is to turn the brief into an executable baseline implementation that already adheres to the required API, I/O policy, determinism, and output schema (with \textbf{CGA} executing \texttt{code}-\texttt{generation} prompt).

At \emph{iteration} \emph{\(t\)}, we use \textbf{SEA} to perform the \emph{forward execution}:
\[
o_t = f_{\mathrm{Sim}}(x_t, I).
\]
Here, the \emph{input} is the current simulator code \(x_t\) and the evaluation inputs \(I\) (validation data). The \emph{output} is the simulator outputs \(o_t\) (e.g., trajectories, curves, logs, intermediate traces). The \emph{job} of this mapping is to compile/run \(x_t\) on \(I\), producing the observables needed for scoring; it also yields run metadata (errors, timing, determinism checks) that is later used as evidence for feedback.

After the forward computation, we employ \textbf{REA} to compare the simulator’s predictions against the ground-truth observables to compute the \emph{loss}:
\[
L_t = \ell(o_t, Y) + \lambda \sum_{j} \max\!\bigl(0, c_j(x_t)\bigr).
\]
The \emph{input} is the simulator outputs \(o_t\) and the ground-truth observables \(Y\). The \emph{output} is a scalar loss \(L_t\) (lower is better). The \emph{job} of this mapping is to measure how closely the simulator matches reality, e.g., via MSE/MAE over curves, distributional distances (JS), or task-specific metrics.

In parallel, we use \textbf{REA} to enforce \emph{constraint satisfaction}: throughout, we require \(x_t \in \mathcal{C}\) (no syntax errors; compilable; policy-compliant I/O; non-empty main flow; output schema conformity; etc.). Violations are both \emph{forbidden} for the final solution and \emph{used as evidence} in the backward step.

\paragraph{\textbf{(4) Textual Gradients (Backward as Text)}}

In our graph, \(x_t\) has one numeric successor (\emph{``simulate \& score''}). Therefore, by the chain rule, we have:
\[
\frac{\partial L_t}{\partial x_t}
=
\frac{\partial L_t}{\partial o_t}
\cdot
\frac{\partial o_t}{\partial x_t}
=
\nabla_{\mathrm{LLM}}(x_t, o_t, \tfrac{\partial L_t}{\partial o_t}).
\]
Here, we use \(\nabla_{\mathrm{LLM}}\) to compose natural-language feedback such as ``\emph{This prediction can be improved by \dots}'' where the feedback \emph{describes how to modify the variable} to improve the downstream objective, \emph{analogous to gradients} in standard Stochastic Gradient Descent (SGD)~\cite{li2018learning}.

We construct evidence \(\tfrac{\partial L_t}{\partial o_t}\) to describe the criticisms on the \emph{prediction} $o_t$ (completed by the \textbf{FGA} using the \texttt{output}-\texttt{criticism} prompt.): \emph{diffs} between \(o_t\) and \(Y\) revealed by evaluation metrics, and \emph{constraint violations} \(\{c_j(x_t) > 0\}\) with failing tests (e.g., compile errors, IO errors, abnormal outputs discovered during simulator execution).
Then, we have:
\begin{align}
g_t \;\triangleq\; \frac{\partial L_t}{\partial x_t}
&= \nabla_{\mathrm{LLM}}\!\left(x_t, o_t, \tfrac{\partial L_t}{\partial o_t}\right) \\
&\triangleq\; \mathrm{LLM}\Big(
   \text{We run simulator $x_t$ and obtain output $o_t$:} \nonumber \\
& \quad \;\;\{o_t \mid x_t\}. \nonumber \\
& \quad \;\;\text{Below are the critiques on $o_t$: }
   \big\{\tfrac{\partial L_t}{\partial o_t}\big\}. \nonumber \\
& \quad \;\;\text{Explain how to improve $x_t$.}\Big)
\end{align}
The resulting \emph{textual gradient} is \emph{a set of localized, actionable code-edit patches}.


\paragraph{\textbf{(5) Textual Momentum}}
In standard SGD, momentum (Polyak Heavy-Ball)~\cite{scieur2020universal} uses a linear combination of past gradients and the most recent one to define a new gradient for updating a variable. 
Analogously, to \emph{stabilize long-horizon editing}, we maintain a momentum buffer \(m_t\) as an \emph{exponentially decayed synopsis} of past critiques:
\[
m_t = \mathrm{Decay}_{\beta}(m_{t-1}) \;\oplus\; g_t,
\]
where \(\oplus\) denotes \emph{ordered merge}, and \(\mathrm{Decay}_{\beta}\) down-weights stale items (keep last $K$ iterations).

Concretely, we \emph{keep track of past gradients} by maintaining a \emph{historic log} \(\{M\}\) that records the optimization history across iterations. 
After each code optimization round, we append the current gradient to the tail of \(\{M\}\). 
When forming the current \textbf{Textual Momentum}, we use \(\mathrm{Decay}_{\beta}(m_{t-1})\) to retrieve the \emph{latest} \emph{$K$} (in our implementation $K=3$) historical gradient records from \(\{M\}\), and we \emph{extract salient edits/themes} from them to understand: (1) \emph{what mistakes} prior code versions made (to avoid repeating them); (2) \emph{how we previously fixed issues} (to inform the current round). We then merge \(\mathrm{Decay}_{\beta}(m_{t-1})\) with the \emph{current} detailed code-edit feedback \(g_t\) into \(m_t\), which acts as the \emph{refined gradient}.

Our Momentum buffer—which summarizes prior critiques together with the current feedback—plays the same memory/reflection role as in Reflexion~\cite{shinn2023reflexion} and the iterative self-feedback role in Self-Refine~\cite{madaan2023self}. 
By conditioning the next update on history rather than only the latest signal, it operationalizes exactly the mechanism these methods credit for outperforming one-shot prompting. 
In our design, \textbf{momentum} enriches the optimizer’s context, enabling progressively smaller, better-aligned edits over time and reducing the chance of repeating past mistakes.
Here, the \textbf{FGA}, loaded with the \texttt{gradient}-\texttt{generation} prompt, is responsible for generating the \emph{textual gradients} and \emph{momentum-based} summarization.

\paragraph{\textbf{(6) Projected Gradient Descent (PGD)}}
In classical PGD~\cite{agarwal2010fast,chen2015fast}, each gradient step is followed by a projection \(\Pi_{\mathcal{C}}\) (mapping \(z\) to a point in the feasible set \(\mathcal{C}\)); analogously, \socia implements a textual analogue of \textbf{PGD}.

Specifically, we employ \textbf{Textual Momentum} to perform \emph{textual gradient descent–based optimization} and \emph{variable updates}, we have:
\begin{align}
x_{t+1}^{\mathrm{unproj}}
&= \mathrm{TGD.step}(x_t, m_t; r) \nonumber\\
&\triangleq\;
\mathrm{LLM}(
\begin{aligned}[t]
&\text{We have critiques on }\{x_t\}\text{: }\{m_t\}\text{.}\\
&\text{Incorporate them to optimize code.)}
\end{aligned}
\end{align}

Here, \texttt{TGD.step} receives: (i) the current \(x_t\); (ii) the aggregated critiques \(m_t\); (iii) the role description \(r\), and returns the \emph{corrected code} \(x_{t+1}^{\text{unproj}}\).
Here we use \textbf{CGA} to execute \texttt{code}-\texttt{optimization} prompt to edit code.

Afterwards, we \emph{project} \(x_{t+1}^{\text{unproj}}\) back to the feasible set using a \textbf{textual projector} \(\Pi_{\mathcal{C}}\) that repairs violations via the \emph{smallest necessary edits}:
\[
x_{t+1} = \Pi_{\mathcal{C}}(x_{t+1}^{\text{unproj}}), \qquad
\Pi_{\mathcal{C}}: \mathcal{T} \rightarrow \{\,x:\; c_j(x)\le 0\ \forall j\,\}.
\]
\emph{Practically}, \(\Pi_{\mathcal{C}}\) is designed as a \emph{constraint repairer} that sequentially performs \emph{static checks}, \emph{interface tests}, \emph{compilation checks}, etc.; if a violation is detected, it conducts \emph{minimal-edit repairs} (an inner loop of \textbf{CGA}'s \emph{code-fix} \(\leftrightarrow\) \emph{self-check}; up to \emph{three} attempts per iteration). We write the constraint rules into \texttt{<CONSTRAINTS>} in the \textbf{CGA}'s \texttt{code}-\texttt{fix} prompt so that they become the target of the projector.

\paragraph{\textbf{(7) One-Line Summary (All Pieces Together)}}

\begin{simstepbox}
\begin{tabularx}{\linewidth}{@{}l X@{}}

\textbf{Forward:} &
\(
\begin{aligned}[t]
o_t &= f_{\mathrm{Sim}}(x_t, I),\\
L_t &= \ell(o_t, Y) + \lambda \sum_{j} \max\!\bigl(0, c_j(x_t)\bigr).
\end{aligned}
\)\\[4pt]

\textbf{Backward:} &
\( g_t = \nabla_{\mathrm{LLM}}(x_t, o_t, \tfrac{\partial L_t}{\partial o_t}) \)\\[4pt]

\textbf{Momentum:} &
\( m_t = \mathrm{Decay}_{\beta}(m_{t-1}) \oplus g_t \)\\[4pt]

\textbf{Update:} &
\(
\begin{aligned}[t]
x_{t+1}^{\text{unproj}} &= \mathrm{TGD.step}(x_t, m_t; r),\\
x_{t+1} &= \Pi_{\mathcal{C}}\!\left(x_{t+1}^{\text{unproj}}\right).
\end{aligned}
\)\\
\end{tabularx}
\end{simstepbox}



We iteratively optimize \(x\), and \emph{stop by early-stopping on validation} when \(L_t\) \emph{plateaus} and \emph{all constraints} hold.










==> latex/chapter/4_exp_setup_old.tex <==
\subsection{Benchmarks}
We evaluate \socia on three real-world–inspired simulation tasks.
% , each grounded in one CPS (\textit{cyber, physical, or social}) dimension:

     \paragraph{\textbf{(1) User Modeling}} (\textit{cyber} space, \textit{agent-based} model), drawn from the AgentSociety Challenge~\cite{DBLP:journals/corr/abs-2502-18754}, uses an LLM as a tool to predict ratings for new products from users’ historical star ratings on an e-commerce platform.
    
     \paragraph{\textbf{(2) Mask Adoption Behavior Simulation}} (\textit{social} space, \textit{aggregate} model), models the temporal dynamics of mask-wearing decisions during a pandemic in a socially embedded population. Decisions depend on heterogeneous social ties, risk perception, and governmental interventions, with a public-health campaign on Day~10 triggering diffusion. Inspired by the data paradigms in BESSIE~\cite{DBLP:journals/corr/abs-2203-11414} and pandemic-era mask decision simulators~\cite{mitsopoulos2023masking}, we generate manually perturbed, LLM-based synthetic data for 1{,}000 agents embedded in a multi-relational graph; \textit{note}: from Day~10 onward, an external governmental intervention affects community decisions, and the simulator must model this intervention process.
    
    \paragraph{\textbf{(3) Personal Mobility Generation}} (\textit{physical} space, \textit{agent-based} model), adopts the LLMob dataset~\cite{wang2024large} containing real-world spatiotemporal trajectories from residents in Japan. The objective is to predict each individual’s next-day mobility trajectory under three settings: (a) normal $\rightarrow$ normal, (b) pandemic $\rightarrow$ pandemic, and (c) normal $\rightarrow$ pandemic using only normal-period history. \textit{Note}: \textbf{Personal Mobility} includes both in-domain (ID) fitting (normal$\rightarrow$normal and pandemic$\rightarrow$pandemic; training and prediction data follow the same distribution) and out-of-domain (OOD) extrapolation (normal$\rightarrow$pandemic), requiring the simulator to generalize to new conditions to answer “\textbf{what-if}” questions.

\subsection{Baseline Methods.}
We compare \socia against several baselines.\textbf{AI Scientist-v2}~\cite{yamada2025ai} is an automated pipeline that ingests experimental data and constructs/executes ML-based models; however, due to the complexity of simulator construction, AI Scientist-v2 still requires a certain amount of \textit{manual} code adjustments to complete code generation.

We also include \textbf{YuLan-OneSim}~\cite{wang2025yulan}, which structures scenarios via the ODD protocol~\cite{grimm2010odd}, generates code with a Behavior Graph, and improves it via an iterative \emph{verify–repair–regenerate} loop; \textit{note}: YuLan-OneSim provides scenario-aware data understanding (metrics, analysis, and real/Sim alignment) for its simulations, but it is not a general-purpose data-understanding or statistical calibration toolkit. Therefore, for fairness, we equip it with \socia’s data-understanding module in our implementation.

The \textbf{G-SIM} family~\cite{DBLP:journals/corr/abs-2506-09272} is another key baseline: it uses LLMs to generate simulator code and integrates gradient-free calibration, including evolutionary strategies (\textbf{G-SIM-ES}) and simulation-based inference (\textbf{G-SIM-SBI}), to produce calibrated, uncertainty-aware simulators; G-SIM-SBI offers stronger OOD extrapolation.

Also, we compare with \textbf{Reflexion}~\cite{shinn2023reflexion}, which prompts an LLM to self-reflect on code snippets, writes verbal reflections from trial feedback and stores them in episodic memory to guide subsequent trials, and—conditioned on these reflections and observed errors—produces updated code.
In our implementation, all other mechanisms mirror \socia, except that Reflexion’s self-check/self-update is used to refine simulator code.

\subsection{Evaluation metrics and Implementation.}
\textbf{Evaluation metrics.}
We report \textbf{means with 95\% confidence intervals}. Stochastic LLM- and simulator-based runs are repeated with five seeds~\cite{colas2018many}, while SBI draws $1{,}000$ posterior samples to propagate parameter uncertainty~\cite{falkiewicz2023calibrating}.
Task-specific metrics (following \textbf{CoT}-structured prompts, see \S\ref{ssec:agent}) are:
\textbf{MAE} for \textbf{User Modeling}~\cite{DBLP:conf/naacl/WangJCYZCFLHY24};
\textbf{RMSE} for \textbf{Mask Adoption}, emphasizing large deviations; and
\textbf{DARD}/\textbf{STVD} for \textbf{Personal Mobility Generation}, measuring activity–time and spatiotemporal footprint alignment.
All are error distances, where \textbf{lower} $\downarrow$ indicates \textbf{better} $\uparrow$ performance.

\textbf{Implementation.}
All \socia agents—and the reproduced baselines—are built on GPT-5~\citep{openai2025gpt5}.
We re-implemented baselines either via code reproduction or via dataset-level reproduction to ensure evaluation consistency.



==> latex/chapter/ack.tex <==
GPT-5.2 was used as the backbone language model for the agents in \socia and for the experiments reported in this paper. 
ChatGPT was also used for language polishing and grammar correction during manuscript preparation. 
The authors reviewed, verified, and take full responsibility for all technical content, experimental results, analyses, citations, and final manuscript text.

==> latex/resources/alg_workflow_textgrad.tex <==
\begin{algorithm}[!htbp]
\caption{\socia Pipeline}
\label{alg:sociaworkflow}
\begin{algorithmic}[1]

\State \textbf{Inputs:} Full dataset $D$, task description $T$, role
description $r$, task inputs $I$, observed targets $Y$, hard constraints
$\mathcal C$, tolerance $\varepsilon_{\mathrm{improve}}>0$, maximum
outer-loop budget $T_{\max}$

\State \textbf{Output:} Best feasible simulator program $x^\ast$

\Statex
\State \textbf{Initialization}

\State $D_s \gets \textsc{BuildDataSchema}(D,T,I)$

\State $\mathcal B \gets \textsc{DAA}(D_s,T)$
\Comment{Construct grounded simulator blueprint.}

\State $\boldsymbol{\mu}^{\star}
\gets \textsc{ReferenceMetrics}(Y)$
\Comment{Compute reference metric values from observations.}

\State $x_0 \gets f_{\mathrm{CGA}}(\mathcal B,r)$
\Comment{Synthesize initial executable simulator.}

\State $\text{best\_L} \gets +\infty,\quad
       \text{best\_x} \gets \mathrm{None}$

\State $t \gets 0,\quad
       \text{no\_improve} \gets 0,\quad
       m_{-1} \gets \emptyset$

\Statex
\State \textbf{Diagnosis-Driven Textual-Gradient Refinement Loop}

\While{$t<T_{\max}$}

    \State $(o_t,e_t) \gets f_{\mathrm{SEA}}(x_t,I)$
    \Comment{Execute simulator and collect outputs and execution evidence.}

    \State $\boldsymbol{\mu}_t
    \gets \textsc{Metrics}(o_t,Y)$

    \State $\mathbf r_t
    \gets
    \mathrm{Residual}
    (\boldsymbol{\mu}_t,\boldsymbol{\mu}^{\star})$
    \Comment{Preserve metric-level behavioral residuals.}

    \State $v_t
    \gets
    \textsc{ConstraintReport}(x_t,\mathcal C)$

    \State $L_t
    \gets
    \ell(o_t,Y)
    +
    \lambda\sum_j\max\!\bigl(0,c_j(x_t)\bigr)$

    \State $d_t
    \gets
    \mathcal D_{\mathrm{LLM}}
    (x_t,\mathbf r_t,\mathcal B,e_t,v_t)$
    \Comment{Ground residuals to mechanisms and supported contexts.}

    \State $g_t
    \gets
    \mathcal G_{\mathrm{LLM}}
    (x_t,\mathbf r_t,d_t,e_t,v_t)$
    \Comment{Convert grounded diagnosis into localized textual repair.}

    \State $m_t
    \gets
    \mathrm{Decay}_{\beta}(m_{t-1})
    \oplus
    g_t$
    \Comment{Aggregate repair signal with recent history.}

    \State $\tilde{x}_{t+1}
    \gets
    \mathrm{TGD.step}(x_t,m_t;r)$
    \Comment{Apply mechanism-level code repair.}

    \State $x_{t+1}
    \gets
    \Pi_{\mathcal C}(\tilde{x}_{t+1})$
    \Comment{Repair updated simulator to satisfy hard constraints.}

    \Statex
    \Comment{--- Incumbent tracking and early stopping ---}

    \If{$x_t\in\mathcal C$
        \textbf{and}
        $L_t<\text{best\_L}-\varepsilon_{\mathrm{improve}}$}

        \State $\text{best\_L}\gets L_t$
        \State $\text{best\_x}\gets x_t$
        \State $\text{no\_improve}\gets 0$

    \Else

        \State $\text{no\_improve}
        \gets
        \text{no\_improve}+1$

        \If{$\text{no\_improve}\geq2$}
            \State \Return $\text{best\_x}$
            \Comment{Stop after two rounds without sufficient improvement.}
        \EndIf

    \EndIf

    \State $t\gets t+1$

\EndWhile

\State \Return $\text{best\_x}$

\end{algorithmic}
\end{algorithm}


==> latex/table/simulation_code_iteration.tex <==
\begin{table*}[h]
    % \caption{Summary of differences between \libName and other related multi-agent systems.  \textbf{infrastructure}: whether the system is designed as a generic infrastructure for building LLM applications. \textbf{conversation pattern}: the types of patterns supported by the implemented systems. Under the `static’ pattern, agent topology remains unchanged regardless of different inputs. \libName allows flexible conversation patterns, including both static and dynamic patterns that can be customized based on different application needs.  
    % \textbf{execution-capable}: whether the system can execute LLM-generated code; \textbf{human involvement}: whether (and how) the system allows human participation during the execution process of the system. \libName allows flexible human involvement in multi-agent conversation with the option for humans to skip providing inputs. 
    % }
    \caption{
    Summary of the functionalities achieved by the generated code at different stages (\textbf{iterations}) across various applications. \textbf{Blank cells} in the table indicate functionalities that \textbf{were not successfully implemented}.
    In terms of naming of \textbf{Code}, the format follows \textbf{Application-Number}, such as ``User-0'', which represents the simulator generated for the \textit{User Modeling Task} at \textit{}{Iteration 0}.
    }
    \label{tab:simulation_code_iteration}
    \small
        \begin{tabular}{p{1.4cm}|P{1.66cm}P{1.66cm}P{1.66cm}P{1.66cm}P{1.66cm}P{1.66cm}}
            \hline %\hline
           Code & Writing component classes & Building the simulator framework & Error Handling & Visuali-zation  & Parameter calibration & Model refinement  \\ \hline
            User-0 & \cmark &   &  &     &  &   \\
            User-1 & \cmark & \cmark  &  &     &  &   \\
            User-2 & \cmark & \cmark  & \cmark &     &  &   \\
            User-3 & \cmark & \cmark  & \cmark & \cmark    &  &   \\
            User-4 & \cmark & \cmark  & \cmark &  \cmark   & \cmark &   \\
            User-5 & \cmark & \cmark  & \cmark &  \cmark   & \cmark & \cmark  \\
            \hline
            Mobility-0 & \cmark & \cmark  &  &     &  &   \\
            Mobility-1 & \cmark & \cmark  & \cmark &  \cmark   &  &   \\
            Mobility-2 & \cmark & \cmark  & \cmark &  \cmark   & \cmark &   \\
            Mobility-3 & \cmark & \cmark  & \cmark &  \cmark   & \cmark & \cmark  \\
            \hline
            Mask-0 & \cmark & \cmark  &  &     &  &   \\
            Mask-1 & \cmark & \cmark  & \cmark &     &  &   \\
            Mask-2 & \cmark & \cmark  & \cmark &  \cmark   &  &   \\
            Mask-3 & \cmark & \cmark  & \cmark &  \cmark   &  &   \\
            Mask-4 & \cmark & \cmark  & \cmark &  \cmark   & \cmark &   \\
            Mask-5 & \cmark & \cmark  & \cmark &  \cmark   & \cmark & \cmark  \\
            \hline
        \end{tabular}
\end{table*}
